In The Wild Ellipse Parameter Estimation for Circular Dining Plates and Bowls

Ellipse estimation is an important topic in food image processing because it can be leveraged to parameterize plates and bowls, which in turn can be used to estimate camera view angles and food portion sizes. Automatically detecting the elliptical rim of plates and bowls and estimating their ellipse parameters for data "in-the-wild" is challenging: diverse camera angles and plate shapes could have been used for capture, noisy background, multiple non-uniform plates and bowls in the image could be present. Recent advancements in foundational models offer promising capabilities for zero-shot semantic understanding and object segmentation. However, the output mask boundaries for plates and bowls generated by these models often lack consistency and precision compared to traditional ellipse fitting methods. In this paper, we combine ellipse fitting with semantic information extracted by zero-shot foundational models and propose WildEllipseFit, a method to detect and estimate the elliptical rim for plate and bowl. Evaluation on the proposed Yummly-ellipse dataset demonstrates its efficacy and zero-shot capability in real-world scenarios.

==> figs/bottom.tex <==
% Use figure* for multi-column figure
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{bottom.png}
    \caption{Image illustrating the process used to ignore bottom bowl edges. Two bounding boxes, the blue one representing food and the red representing the closest bowl bounding box. The green line is the distance from the bottom of the food bounding box to the lowest point on the contour within that gap.}
    \label{fig:bottom}
\end{figure}


==> figs/diagram.tex <==
% https://q.uiver.app/#q=WzAsNixbMiw3LCJQX3tpfSJdLFsxMiwxLCJQX3tpK3N9Il0sWzIzLDAsIlBfe2krMnN9Il0sWzI3LDEsIlxcYnVsbGV0Il0sWzAsMTEsIlxcYnVsbGV0Il0sWzE4LDJdLFsxLDIsIiIsMix7ImN1cnZlIjotMiwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDEsIiIsMix7ImN1cnZlIjotNSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDEsIkRfe2l9IiwyLHsiY29sb3VyIjpbMCw2MCw2MF19LFswLDYwLDYwLDFdXSxbMSwyLCJEX3tpKzF9IiwyLHsiY29sb3VyIjpbMCw2MCw2MF19LFswLDYwLDYwLDFdXSxbMiwzLCIiLDIseyJjdXJ2ZSI6LTF9XSxbNCwwLCIiLDIseyJjdXJ2ZSI6LTF9XV0=
\begin{figure}
\begin{adjustbox}{width=\linewidth}
\begin{tikzcd}
	&&&&&&&&&&&&&&&&&&&&&&& {P_{i+2s}} \\
	&&&&&&&&&&&& {{P_{i+s}}} &&&&&&&&&&&&&&& \bullet \\
	&&&&&&&&&&&&&&&&&& {} \\
	\\
	\\
	\\
	\\
	&& {P_{i}} \\
	\\
	\\
	\\
	\bullet
	\arrow[curve={height=-12pt}, no head, from=2-13, to=1-24]
	\arrow[curve={height=-30pt}, no head, from=8-3, to=2-13]
	\arrow["{D_{i}}"', color={rgb,255:red,214;green,92;blue,92}, from=8-3, to=2-13]
	\arrow["{D_{i+1}}"', color={rgb,255:red,214;green,92;blue,92}, from=2-13, to=1-24]
	\arrow[curve={height=-6pt}, from=1-24, to=2-28]
	\arrow[curve={height=-6pt}, from=12-1, to=8-3]
\end{tikzcd}
\end{adjustbox}
\end{figure}

==> figs/diagram2.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/diagram2.png}
    \caption{Visualization of $\Vec{D}$}
    \label{fig:curvediagram}
\end{figure*}

==> figs/diagram3.tex <==
\begin{figure}
\begin{adjustbox}{width=0.89\linewidth}
\centering
\input{figs/ellipse-diagram.tikz}
% \tikz[baseline=-0.5em]{\node[draw=red,font=\color{red},fill=red!10!white]{ }}
\end{adjustbox}
\caption{A visual representation of distance vectors $d$ drawn between each point $p \in P$.}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

